VisIT-Bench: A Benchmark for Vision-Language Instruction Following Inspired by Real-World Use

We introduce VisIT-Bench (Visual InsTruction Benchmark), a benchmark for evaluation of instruction-following vision-language models for real-world use. Our starting point is curating 70 'instruction families' that we envision instruction tuned vision-language models should be able to address. Extending beyond evaluations like VQAv2 and COCO, tasks range from basic recognition to game playing and creative generation. Following curation, our dataset comprises 592 test queries, each with a human-authored instruction-conditioned caption. These descriptions surface instruction-specific factors, e.g., for an instruction asking about the accessibility of a storefront for wheelchair users, the instruction-conditioned caption describes ramps/potential obstacles. These descriptions enable 1) collecting human-verified reference outputs for each instance; and 2) automatic evaluation of candidate multimodal generations using a text-only LLM, aligning with human judgment. We quantify quality gaps between models and references using both human and automatic evaluations; e.g., the top-performing instruction-following model wins against the GPT-4 reference in just 27% of the comparison. VisIT-Bench is dynamic to participate, practitioners simply submit their model's response on the project website; Data, code and leaderboard is available at visit-bench.github.io.

==> sections/6_related_work.tex <==
Our work is related to previous work on multimodal models for image-text understanding, instruction-following, and benchmarking in machine learning. We provide a detailed overview of related work in \S \ref{sec:related-appendix}. Multi-model modals for image-text understanding have recently emerged as powerful and useful methods for many image-language reasoning tasks \cite{Alayrac2022FlamingoAV, li2023blip, liu2023llava, pandey2022cross, su2023pandagpt, dai2023instructblip, ye2023mplug, anas_awadalla_2023_7733589, gpt4}. Both language and multimodal models are often trained to follow language instruction, a paradigm known as ``instruction following'' \cite{alpaca, gao2023llama, koala_blogpost_2023, dai2023instructblip, liu2023llava, ye2023mplug}. Despite the success of these approaches on existing vision-language datasets (GQA, Image Captioning \cite{antol2015vqa,hudson2019gqa,lin2014microsoft}), there is a lack of a high-quality benchmarking dataset for multimodal instruction-following tasks that reliably replicates the way in which humans would interact with multimodal chatbots in the wild. This lack of benchmarking data makes reliable assessments of progress difficult \cite{liao2021we}, and has contributed to a lack of empirical evaluations of instruction-following models.


==> sections/99_checklist.tex <==
%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNo{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/old/4_eval_benchmark.tex <==
The aim of \benchmarkname is to devise a robust and accurate automatic evaluation methodology for vision and language (V\&L) chatbots that reflect real-world usage. We start this process by accumulating human annotations through pairwise model comparisons, thus establishing a baseline of human-rated model performance. The human annotation serves as the key benchmark against which we later assess different automatic evaluation metrics, the objective being to find the metric that mirrors human judgement most accurately. 

\subsection{Model Setup}

The setup for our vision-language baselines is twofold. For two-stream models, we use the image as input for the vision encoder and the instruction as a prompt for the text encoder. On the other hand, in-context single-stream models take a concatenated image and instruction as inputs. Execution-based models, such as VisualChatGPT~\cite{wu2023visual}, implement a chat window for each sample, holding inputs and intermediate chains of thoughts and actions in memory. Subsequently, the image and instruction are fed to the model in sequence. Each model's inputs and outputs are meticulously described, noting the origins when applicable, such as human-generated dense captions or model outputs drawn from GPT.

\paragraph{Evaluated Models} Our evaluation utilises a selection of publicly accessible vision-language models that have been fine-tuned with multimodal instructions. These models include LLaVA-13B~\cite{liu2023visual}, InstructBLIP-13B~\cite{dai2023instructblip}, Multimodal GPT~\cite{gong2023multimodal}, MiniGPT4~\cite{zhu2023minigpt}, OpenFlamingo~\cite{anas_awadalla_2023_7733589}, Otter~\cite{li2023otter}, mPlugOwl~\cite{ye2023mplug}, LlamaAdapterv2~\cite{gao2023llama}, PandaGPT-13B~\cite{su2023pandagpt}, VisualChatGPT~\cite{wu2023visual}.

\hritik{Adding the structure for the experiments section -- subject to changes}

\subsection{Human Annotation and Model Ranking}

We leverage human annotation as a primary tool for benchmarking model performance and guiding the design of our automatic evaluation.

We collect 1,000 pairwise model rankings through crowdsourcing, where annotators are given an image, an instruction, and responses from two different models (Model A and Model B). Their task is to discern the superior model, based on the criteria of instruction adherence, factual accuracy, helpfulness, and detailed response.

The results, presented in \Cref{tab:table_human_scoring_results}, offer a snapshot of model performance from the human perspective, which is instrumental in bridging the evaluation gap for models lacking sufficient assessment.

These findings serve as a cornerstone for our subsequent efforts in devising a fitting automatic evaluation metric.

\begin{table}[h]
\centering
\caption{Human Scoring Results}
\label{tab:table_human_scoring_results}
\begin{tabular}{lc}
\toprule
\textbf{Model} & \textbf{Score} \\
\midrule
Human Verified Reference \hritik{why not just say GPT-4?} & 0.845 \\
LLaVA-13B & 0.635 \\
mPLUG-Owl & 0.593 \\
InstructBLIP-13B & 0.472 \\
LlamaAdapter-v2 & 0.461 \\
MiniGPT-4 & 0.337 \\
PandaGPT-13B & 0.220 \\
\bottomrule
\end{tabular}
\end{table}

